Distributed and Autonomic Minimum Spanning Trees

The most common strategy for enabling a process in a distributed system to broadcast a message is one-to-all communication. However, this approach is not scalable, as it places a heavy load on the sender. This work presents an autonomic algorithm that enables the $n$ processes in a distributed system to build and maintain a spanning tree connecting themselves. In this context, processes are the vertices of the spanning tree. By definition, a spanning tree connects all processes without forming cycles. The proposed algorithm ensures that every vertex in the spanning tree has both an in-degree and the tree depth of at most $log_2 n$. When all processes are correct, the degree of each process is exactly $log_2 n$. A spanning tree is dynamically created from any source process and is transparently reconstructed as processes fail or recover. Up to $n-1$ processes can fail, and the correct processes remain connected through a scalable, functioning spanning tree. To build and maintain the tree, processes use the VCube virtual topology, which also serves as a failure detector. Two broadcast algorithms based on the autonomic spanning tree algorithm are presented: one for best-effort broadcast and one for reliable broadcast. Simulation results are provided, including comparisons with other alternatives.

==> sections/VCubeSurvey.tex <==
\subsection{A Survey on the VCube \& Applications}

VCube was originally proposed in the context of system-level diagnosis \cite{masson1996system}. The first system-level diagnosis model was published in 1967, Preparata, Metze and Chien \cite{pmc:1967} and called the PMC model after the author's initials. In the PMC model, the system consists of units that can test each other. A test is a procedure that is complete enough to determine whether the tested unit is \textit{faulty} or \textit{fault-free}. The set of all test results is called the \textit{syndrome} of the system. A central entity external to the system collects and processes the syndrome to classify the units as faulty or fault-free. In 1974, Hakimi and Amim \cite{hakimi1974characterization} proved that for a system of $n$ units to be $t$-diagnosable it is necessary that (i) $n \geq 2t+1$ and that (ii) each process be tested for at least $t$ other processes.

In 1984, two new diagnosis models were proposed that had a major impact on the field. The first model by Hakimi and Nakajima \cite{hakimi1984adaptive} allows the diagnosis to be adaptive, in the sense that the testing assignment is dynamic, i.e., the next tests to be executed are defined according to the results of the previous tests. The other model was proposed by Hosseini, Kuhl, and Reddy \cite{hosseini1984diagnosis}, and eliminated the central entity, allowing for a fully distributed diagnosis.  According to that model, the units not only execute tests, but also collect test results from each other to obtain the syndrome. Each fault-free unit can then process the syndrome and determine the set of faulty units in the system.

In 1992, Bianchini and Buskens \cite{bianchini1992implementation} proposed the combination of adaptive and distributed diagnosis. The Adaptive Distributed System-Level Diagnosis algorithm (Adaptive-DSD) was proposed and used to monitor a large production network. The algorithm is based on a ring topology that presents the optimal number of tests: at most $n$, but the latency is up to $n$ consecutive testing rounds. In 1998, Duarte and Nanya \cite{duarte1998hierarchical} proposed the Hierarchical Adaptive Distributed System-Level Diagnosis algorithm (Hi-ADSD). Hi-ADSD employs a hierarchical virtual topology to organize the system units. Latency is at most $log_2^2 n$ testing rounds, recall that all logarithms in this work are base 2. The Hi-ADSD algorithm was originally proposed for the construction of efficient and fault-tolerant network fault management systems \cite{duarte2002dependable}. 

Hi-ADSD was called VCube for the first time in 2014\cite{duarte2014vcube}. That algorithm presents a testing strategy which guarantees that each process is tested by at 
most $log_2 n$ testers. In the original Hi-ADSD algorithm, there were some rare system configurations in which the number of tests executed could be quadratic. A previous algorithm, Hi-ADSD with Detours \cite{duarte2009hierarquical} also presented a strategy to guarantee a logarithmic number of tests, but the proof of the worst case is still open. VCube also introduced a new feature each correct process executed all its assigned tests at each testing interval (of all $log_2 n$ clusters). Thus VCube provably guarantess that the number of tests executed does not exceed $n log_2 n$ per testing round \cite{duarte2014vcube} .   

The system-level diagnosis results presented above assume the PMC model, and a fully connected system, i.e., the underlying physical topology is a complete graph. There are actually several other models, for instance, those that assume a system of arbitrary topology \cite{duarte2011distributed}, which are partitionable by definition. In these models, the diagnosis problem is actually the problem of computing reachability. Other works consider different diagnosis models. Camargo et al. \cite{camargo2018running} abandoned the assumption of the PMC model by assuming that correct units can make mistakes during tests. Comparison-based diagnostics \cite{duarte:2011,ziwich2016nearly} do not assume crash faults. Faulty units can produce arbitrary outputs. The outputs of multiple units are compared to perform the diagnosis, such as distributed integrity checking \cite{ziwich2005distributed}. Although most models assume that faults are permanent, some approaches have been proposed to diagnose intermittent faults \cite{song2023intermittent, guo2023intermittent}. Finally, the probabilistic diagnosis model also presents an alternative approach, which takes into account the difficulty in defining deterministic tests \cite{blough:1996}.

The system-level diagnosis results presented above assume the PMC model, and a fully connected system, i.e., the topology is a complete graph. There are actually several other models, for instance, those that assume a system of arbitrary topology \cite{duarte2011distributed}, which are partitionable by definition. In these models, the problem of determining which units are faulty becomes the problem of computing the reachability. Other works consider different diagnosis models. Camargo et al. \cite{camargo2018running} abandoned the assumption of the PMC model by assuming that correct units can make mistakes during tests. Comparison-based diagnostics \cite{duarte:2011,ziwich2016nearly} do not assume crash faults. Faulty units can produce arbitrary outputs. The outputs of multiple units are compared to perform the diagnosis, such as distributed integrity checking \cite{ziwich2005distributed}. Although most models assume that faults are permanent, some approaches have been proposed to diagnose intermittent faults \cite{song2023intermittent, guo2023intermittent}. Finally, the probabilistic diagnosis model also presents an alternative approach, which takes into account the difficulty in defining deterministic tests \cite{blough:1996}.


